A recursively feasible and convergent Sequential Convex Programming procedure to solve non-convex problems with linear equality constraints

A computationally efficient method to solve non-convex programming problems with linear equality constraints is presented. The proposed method is based on a recursively feasible and descending sequential convex programming procedure proven to converge to a locally optimal solution. Assuming that the first convex problem in the sequence is feasible, these properties are obtained by convexifying the non-convex cost and inequality constraints with inner-convex approximations. Additionally, a computationally efficient method is introduced to obtain inner-convex approximations based on Taylor series expansions. These Taylor-based inner-convex approximations provide the overall algorithm with a quadratic rate of convergence. The proposed method is capable of solving problems of practical interest in real-time. This is illustrated with a numerical simulation of an aerial vehicle trajectory optimization problem on commercial-of-the-shelf embedded computers.

==> Convexification.tex <==
Now we turn our attention into finding the convex inner approximations, $g_{\text{cvx},i}^{\left(\bm{x}_{e}\right)}$, required to realize a recursively feasible and convergent SCP.
%If a d.c. decomposition of $g_{i}$ is known then the convexification in Eq.~\eqref{eq:cccp} is sufficient as it meets the required Eq.~\eqref{eq:ConvexProp} conditions. If a d.c. decomposition is not known another method is required.
The methods that are available in the literature are based on finding a d.c. decomposition of the non-convex functions $g_{i}$. Once a d.c. representation of $g_{i}$ is found then a convex inner approximation is obtained by linearizing the concave part as shown in Eq.~\ref{eq:cccp}. In this section, we first briefly review the d.c. decomposition methods available in the literature and later, we propose a general and systematic method to obtain convex inner approximations for functions that accept an expansion as a Taylor's series.

\subsection{Finding d.c. decompositions \label{sec:dc}}
It has been shown that d.c. decompositions exist for any twice differentiable function $g\in\mathcal{C}^{2}$  \cite{Hartman1959,Hiriart1985}, but we will see that these decompositions may be hard to obtain or of very little practical use. 

The regularization approach \cite{Hiriart1985,Aleksandrov2012,Dinh2012,Wang2012b,Scutari2014} is a general method where a d.c. decomposition is obtained by using a sufficiently strong convex function $\phi\left(\bm{x}\right)$ such that
\begin{equation}
g_{i}\left(\bm{x}\right)=\underbrace{ \phi\left(\bm{x}\right)}_{c_{i,1}\left(\bm{x}\right)}-\underbrace{\left(\phi\left(\bm{x}\right)-g_{i}\left(\bm{x}\right)\right)}_{c_{i,2}\left(\bm{x}\right)},\text{ for }\bm{x}\in\mathcal{T}
\end{equation}
is d.c.
 
In general $\mathcal{T}\subset\mathbb{R}^{n}$ and $\bm{x}\in\mathcal{T}$ needs to be enforced as a trust region in the optimization problem.
As an example of this regularization approach let's assume that $g_{i}$ is Lipschitz continuous with a constant $L_{g}$. A d.c. representation over $\bm{x}\in\mathbb{R}^{n}$ is then
\begin{equation}
g_{i}\left(\bm{x}\right)=\underbrace{L_{g}\left\lVert\bm{x}\right\rVert^{2}}_{c_{i,1}\left(\bm{x}\right)}-\underbrace{\left(L_{g}\left\lVert\bm{x}\right\rVert^{2}-g_{i}\left(\bm{x}\right)\right)}_{c_{i,2}\left(\bm{x}\right)}.
\end{equation}
Composition rules also exists that allow to express special types of function compositions as d.c. The interested reader is referred to \cite{Hiriart1985,Wang2012b,Scutari2014} for more details.

Sufficiently strong convex functions where the convexity of $c_{i,2}=\phi\left(\bm{x}\right)-g_{i}\left(\bm{x}\right)$ can be proved may be difficult to obtain and if found the d.c. representation might significantly overestimate $g_{i}$ (as dictated by Eq.~\eqref{eq:ConvexProp_geq}) and thus degrade the SCP procedure's rate of convergence.
It is also worth noting that an infinite amount of d.c. decompositions of $g_{i}$ exists an thus we are presented with the question of, which is the best convex inner approximation of $g_{i}$? Convex inner approximations that minimally overestimate $g$ are therefore preferred. 

%sos
An approach that is able to encode our desire the minimally overestimate $g$ is the decomposition of $g_{i}$ into a difference of convex sum-of-squares (sos-convex) polynomials \cite{Ahmadi2017}. If we assume that $g_{i}$ is a polynomial of degree $d_{g}$, and $\bm{z}\left(\bm{x}\right)$ denote a vector of all the monomials of $\bm{x}$ up to degree $d_{z}\geq d_{g}/2$ then its sos decomposition is
\begin{equation}
\underbrace{\bm{z}^{T}\bm{Q}_{g}\bm{z}}_{g\left(\bm{x}\right)}=\underbrace{\bm{z}^{T}\bm{Q}_{1}\bm{z}}_{c_{1}\left(\bm{x}\right)}-\underbrace{\bm{z}^{T}\bm{Q}_{2}\bm{z}}_{c_{2}\left(\bm{x}\right)}
\label{eq:sos}
\end{equation}
with $\bm{Q}_{g}$, $\bm{Q}_{1}$ and $\bm{Q}_{2}$ are symmetric matrices containing the polynomial coefficients. %(also known as Gram matrices).
For the decomposition to be sos-convex and thus d.c., the $\bm{Q}_{1}$ and $\bm{Q}_{2}$ matrices must be positive semi-definite.
\begin{equation}
\begin{rcases}
\bm{Q}_{1}\succeq 0 \Longrightarrow \bm{z}^{T}\bm{Q}_{1}\bm{z}\text{ is sos-convex}\\
\bm{Q}_{2}\succeq 0 \Longrightarrow \bm{z}^{T}\bm{Q}_{2}\bm{z}\text{ is sos-convex}
\end{rcases}\Longrightarrow g\left(\bm{x}\right)=\bm{z}^{T}\bm{Q}_{1}\bm{z}-\bm{z}^{T}\bm{Q}_{2}\bm{z}\text{ is d.c.}
\end{equation}
There are an infinite amount of sos-convex representations and thus in \cite{Ahmadi2017} different methods to optimize the sos-convex decomposition are proposed.  Interestingly enough, finding these optimized sos-convex decompositions  is a semidefinite programming problem (second order cone or linear programming problem with some additional relaxations) \cite{Ahmadi2017}. It is also worth noting that this approach is general, as any function $g_{i}$ can be converted into polynomial form via a Taylor series, and that it is connected to Laserre's approach in which sos-convex relaxations are used to cast non-convex polynomial programing problems as semidefinite programming problems \cite{Lasserre2001,Nie2013}.
Although it can be argued that finding a sos-convex decomposition is a computationally tractable approach, the dimensionality of the resulting semidefinite programming problem dramatically increases with the number of constraints and variables, effectively limiting the applicability of this approach to small problems. 


\begin{comment}
From the proposed optimize approaches introduced in \cite{Ahmadi2017}, the one that has given good results in our experiments is to minimize the maximum eigenvalue, $\lambda_{\mathrm{max}}$, of the $c_{2}$ Hessian, $\bm{H}_{c_{i,2}}$ (\emph{i.e.}, minimizing the curvature of the concave part). Finding the sos-convex decomposition that optimizes this objective results in the following convex programming problem:
\begin{problem*}
	\textbf{$P_{\mathrm{sos}}$. sos-convex decomposition of $g_{i}$}
	\label{prob:sos}
	\begin{align*}
	%Minimize
	\text{minimize: } & \lambda_{\mathrm{max}}\bm{H}_{c_{i,2}} \\
	\text{subject to: } & Q_{i,g}=Q_{i,1}-Q_{i,2} \tag{$P_{\mathrm{sos}}$}\\
	& Q_{i,1}\succeq 0,\quad Q_{i,2}\succeq 0
	\end{align*}
\end{problem*}
\end{comment}






\begin{comment}
Here, we introduce the concept of a \textit{minimal convex inner approximation}, which we denote by $g_{\text{cvx}}^{\star}$, as the convex inner approximation that satisfies
\begin{equation}
g_{\text{cvx}}^{\star}=\text{inf}\left\{g-g_{\text{cvx}}:g_{\text{cvx}}\text{ satisfies Eq.~\eqref{eq:ConvexProp}} \right\}
\end{equation}


Other methods to generate these global convex overestimators which minimize the nonnegative difference $g_{\text{cvx},i}^{\left(\bm{x}_{e}\right)}\left(\bm{x}\right)- g_{i}\left(\bm{x}\right)\geq 0$ may exist, and if applied, would accelerate the SCP's rate of convergence.
\end{comment}

\subsection{Convex inner approximation of the $g_{i}$ Taylor series \label{sec:IC_Taylor}}
We now present an novel technique to obtain a convex inner approximation of a function. This proposed approach is based on a simple convexification of the Taylor series of a function and it is computationally inexpensive and parallelizable.

To simplify the notation of the high-order terms of the Taylor's series let's use a multi-index notation, with an $n$-tuple of non-negative numbers $\mathbb{N}$, denoted by $\alpha$:
\begin{subequations}
\begin{equation}
\alpha=\left(\alpha_{1},\alpha_{2},\ldots,\alpha_{n}\right),\quad \text{ with }\alpha_{i}\in\mathbb{N}
\end{equation}
\begin{equation}
\left\lvert\alpha\right\rvert=\alpha_{1}+\alpha_{2}+\cdots+\alpha_{n}
\end{equation}
\begin{equation}
\alpha!=\alpha_{1}!\alpha_{2}!\cdots\alpha_{n}!
\end{equation}
\begin{equation}
\bm{x}^{\alpha}=x_{1}^{\alpha_{1}}x_{2}^{\alpha_{2}}\cdots x_{n}^{\alpha_{n}}
\end{equation}
\begin{equation}
\partial^{\alpha}g=\frac{\partial^{\left\lvert\alpha\right\rvert}g}{\partial x_{1}^{\alpha_{1}}\partial x_{2}^{\alpha_{2}}\cdots \partial x_{n}^{\alpha_{n}}}
\end{equation}
\end{subequations}
Using a multi-index notation, the Taylor's expansion of the function $g:\mathbb{R}^{n}\rightarrow\mathbb{R}$ is written as:
\begin{equation}
g\left(\bm{x}\right)=\sum_{\left\lvert\alpha\right\rvert=0}^{\infty}{\frac{\partial^{\alpha}g\left(\bm{x}_{e}\right)}{\alpha!}}\delta\bm{x}^{\alpha}.
\end{equation}
If we only write the first three terms a more familiar expression is recovered:
\begin{equation}
g_{i}\left(\bm{x}\right)=g_{i}\left(\bm{x}_{e}\right)+\delta\bm{x}^{T}\nabla g_{i}\left(\bm{x}_{e}\right)+\frac{1}{2}\delta\bm{x}^{T}\bm{H}_{i}\left(\bm{x}_{e}\right)\delta\bm{x}+\ldots
\label{eq:expansion_three_terms}
\end{equation}
where $\bm{H}_{i}$ denotes the Hessian of $g_{i}$.

To obtain a convex inner approximation of $g$ we propose to convexify all the terms corresponding to the derivatives of second order and higher. The Hessian, as a symmetric matrix, can be decomposed with a positive and negative semi-definite parts:
\begin{equation}
\bm{H}=\bm{H}^{+}+\bm{H}^{-}
\end{equation}
\begin{equation}
\bm{H}^{+}\succeq 0,\quad\bm{H}^{-}\preceq 0.
\end{equation}
The positive semi-definite part is recovered using the matrix of eigenvalues $\bm{\Lambda}$ and the matrix of eigenvectors $\bm{W}$ of the Hessian:
\begin{equation}
\bm{H}^{+}=\bm{W}\bm{\Lambda}^{+}\bm{W}^{T},
\end{equation}
%\begin{equation}
%\bm{H}^{-}=\bm{W}\bm{\Lambda}^{-}\bm{W}^{T}
%\end{equation}
where $\bm{\Lambda}^{+}$ is the matrix of eigenvalues containing only the positive ones. 

The higher order terms ($\left\lvert\alpha\right\rvert\ge 2$) of the Taylor series form homogeneous, polynomial forms
\begin{equation}
\sum_{\left\lvert\alpha\right\rvert}\frac{\partial^{\alpha}g\left(\bm{x}_{e}\right)}{\alpha!}\delta\bm{x}^{\alpha}=\bm{A}\delta\bm{x}^{\alpha}=\sum_{j_{1},\ldots,j_{\left\lvert\alpha\right\rvert}=1}^{n}{a_{j_{1},\ldots,j_{\left\lvert\alpha\right\rvert}}\delta x_{j_{1}}\ldots \delta x_{j_{\left\lvert\alpha\right\rvert}}},
\end{equation}
with $\bm{A}\in\mathbb{R}^{n\times n\times \cdots \times n}$ denoting a supersymmetric --- invariant under permutation on any of its indices --- tensor.

If the eigenvalues and eigenvectors of these tensors are available a similar procedure to the one followed to convexify the Hessian could be pursued.
Although the eigenvalues of tensors can be computed using a sum-of-squares and a semmidefinite programming approach \cite{Cui2014} (again showing the connection with sos-convex decompositions and Lasserre's relaxations), the computational cost quickly becomes prohibitive as the order, or number of variables or constraints increases.

Our proposed approach takes a computational efficient route in where a convex overestimation of the higher order terms, $\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha}\right)$, is obtained as follows:
\begin{equation}
\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha}\right)=\sum_{i=1}^{n}\left({\left\lvert a_{\mathrm{diag},i} \delta x_{i}^{\left\lvert\alpha\right\rvert}\right\rvert^{+}+{a_{\mathrm{cvx},i}\left\lvert \delta x_{i}^{\left\lvert\alpha\right\rvert}\right\rvert}}\right)
\end{equation}
The $a_{\mathrm{diag},i}$ coefficient is the element of the tensor's main diagonal associated with $\delta\bm{x}_{i}$,
\begin{equation}
a_{\mathrm{diag},i}=a_{i,\ldots,i}.
\end{equation}
As $\left\lvert \cdot \right\rvert^{+}$ denotes the positive part operator, the expression ${\left\lvert a_{\mathrm{diag},i} \delta x_{i}^{\left\lvert\alpha\right\rvert}\right\rvert^{+}}$ is convex and is an overestimator of the $\bm{A}\delta\bm{x}^{\alpha}$ terms associated with the $\bm{A}$ tensor's main diagonal.

The $a_{\mathrm{cvx},i}$ coefficient is computed as the sum of the absolute value of all the coefficients in $\bm{A}$ associated with $\delta\bm{x}_{i}$ (with the exception of the coefficient in the main diagonal):
\begin{equation}
a_{\mathrm{cvx},i}=\sum_{j_{1},\ldots,j_{\left\lvert\alpha\right\rvert}=1}^{n}
\begin{cases}
0,&\text{if all }j_{1},\ldots,j_{\left\lvert\alpha\right\rvert}\text{ are different than }i\\
0,&\text{if all }j_{1},\ldots,j_{\left\lvert\alpha\right\rvert}\text{ are equal to }i\\
{\left\lvert a_{j_{1},\ldots,j_{\left\lvert\alpha\right\rvert}}\right\rvert},&\text{otherwise}
\end{cases}
\end{equation}
As $a_{\mathrm{cvx},i}\geq 0$ the term $a_{\mathrm{cvx},i}\left\lvert \delta x_{i}^{\left\lvert\alpha\right\rvert}\right\rvert$ is convex and it follows that
\begin{equation}
\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha}\right)\geq\bm{A}\delta\bm{x}^{\alpha}.
\end{equation}
If the coefficients $a_{\mathrm{cvx},i}$ and $a_{\mathrm{diag},i}$ of a particular order, $\left\lvert\alpha\right\rvert$, are denoted by $a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{cvx},i}$ and $a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{diag},i}$, the proposed inner convex approximation of $g$, satisfying the conditions in Eq.~\eqref{eq:ConvexProp}, is
\begin{equation}
g^{\left(\bm{x}_{e}\right)}_{\text{cvx}}\left(\bm{x}\right)=g\left(\bm{x}_{e}\right)+\delta\bm{x}^{T}\nabla g\left(\bm{x}_{e}\right)
+\frac{1}{2}\delta\bm{x}^{T}\bm{H}^{+}\left(\bm{x}_{e}\right)\delta\bm{x}
+\sum_{\left\lvert\alpha\right\rvert=3}^{\left\lvert\alpha\right\rvert=\infty}{\sum_{i=1}^{n}\left({\left\lvert a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{diag},i} \delta x_{i}^{\left\lvert\alpha\right\rvert}\right\rvert^{+}}+{a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{cvx},i}\left\lvert \delta x_{i}^{\left\lvert\alpha\right\rvert}\right\rvert}\right)}.
\label{eq:gcvx}
\end{equation}

\begin{comment}
From this definition it follows that the proposed $\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha}\right)$ is a inner convex approximation of $\bm{A}\delta\bm{x}^{\alpha}$ as
\begin{equation}
\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha}\right)=\sum_{i=1}^{n}{a_{\mathrm{cvx},i}\left\lvert \delta x_{i}^{\left\lvert\alpha\right\rvert}\right\rvert}\geq \sum_{i_{1},\ldots,i_{\left\lvert\alpha\right\rvert}=1}^{n}{a_{i_{1},\ldots,i_{\left\lvert\alpha\right\rvert}}\delta x_{i_{1}}\ldots \delta x_{i_{\left\lvert\alpha\right\rvert}}}=\bm{A}\delta\bm{x}^{\alpha}.
\end{equation}
satisfying Eq.~\eqref{eq:ConvexProp_geq} for the convexification of the high-order terms.

It is easy to show that the proposed convex approximation for the high-order terms is convex.
For an even order, $\left\lvert\alpha\right\rvert$, the following equality is shown:
\begin{equation}
{a_{\mathrm{cvx}}\left\lvert\delta x_{i}^{\left\lvert\alpha\right\rvert}\right\rvert}=a_{\mathrm{cvx}}\delta x_{i}^{\left\lvert\alpha\right\rvert},
\end{equation}
For an odd $\left\lvert\alpha\right\rvert$ the following equality is shown:
\begin{equation}
{a_{\mathrm{cvx}}\left\lvert\delta x_{i}^{\left\lvert\alpha\right\rvert}\right\rvert}=\begin{cases}
a_{\mathrm{cvx}}\delta x_{i}^{\left\lvert\alpha\right\rvert}, & \text{for }\delta x_{i}\geq 0\\
-a_{\mathrm{cvx}}\delta x_{i}^{\left\lvert\alpha\right\rvert}, & \text{for }\delta x_{i}< 0
\end{cases}
\end{equation}
The $\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha}\right)$ expression, being a sum of convex terms, is convex and thus satisfies Eq.~\eqref{eq:ConvexProp_cvx}.

If the coefficient $a_{\mathrm{cvx}}$ of a particular order, $\left\lvert\alpha\right\rvert$, is denoted by $a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{cvx}}$, the proposed convex approximation of $g$, satisfying the conditions in Eq.~\eqref{eq:ConvexProp}, is
\begin{equation}
g^{\left(\bm{x}_{e}\right)}_{\text{cvx}}\left(\bm{x}\right)=g\left(\bm{x}_{e}\right)+\delta\bm{x}^{T}\nabla g\left(\bm{x}_{e}\right)
+\frac{1}{2}\delta\bm{x}^{T}\bm{H}^{+}\left(\bm{x}_{e}\right)\delta\bm{x}
+\sum_{\left\lvert\alpha\right\rvert=3}^{\left\lvert\alpha\right\rvert=\infty}{\sum_{i=1}^{n}{a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{cvx}}\left\lvert \delta x_{i}^{\left\lvert\alpha\right\rvert}\right\rvert}}.
\label{eq:gcvx}
\end{equation}
\end{comment}

\begin{comment}
\subsubsection{truncating the series}
The proposed convex inner approximation is tight until 

\begin{equation}
\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha}\right)-\bm{A}\delta\bm{x}^{\alpha}\geq s\geq 0
\end{equation}
We are interested in knowing when the overestimation is minimal, i.e, what is  $\min\left(s\right)$ and when does it occur.
Let's assume a worst case scenario when $\delta\bm{x}_{i}$ associated with the smallest $a_{\mathrm{cvx},i}$ is the only $\delta\bm{x}_{i}\neq 0$
\begin{equation}
\delta\bm{x}_{m}=t\geq 0 
\end{equation}
Let's also assume that
\begin{equation}
a_{j_{1},\ldots,j_{\left\lvert\alpha\right\rvert}}\geq 0
\end{equation}
then the elements of the main diagonal are correctly computed.

The off diagonal elements are overestimated as they would otherwise be zero.
\begin{equation}
a_{\mathrm{cvx},m}t^{\left\lvert\alpha\right\rvert}=s
\end{equation}
To keep our promise
\begin{equation}
a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{over}}t^{\left\lvert\alpha\right\rvert}\geq
\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha}\right)-\bm{A}\delta\bm{x}^{\alpha}\geq s\geq 0
\end{equation}
\end{comment}



\subsection{Truncating the series}\label{sec:trust_regions}
The inclusion of high order terms may need to be truncated as the Taylor's series may be infinite or the amount of effort required to compute high-order terms too computationally expensive. We now present a trust-region based method that allows to truncate the series while retaining the convex inner approximation property.

The idea is to define a trust region
\begin{equation}
\left\lVert \delta\bm{x}\right\rVert_{2} \leq \rho,
\end{equation}
where the convex inner approximation property can be guaranteed up to a certain level. In particular we are interested in showing that within the trust region
\begin{equation}
\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha}\right)-\bm{A}\delta\bm{x}^{\alpha}\geq \bm{A}\delta\bm{x}^{\alpha+1}\leq\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha+1}\right)
\end{equation}
If we let $s^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{min}}$ denote the smallest overestimation
\begin{equation}
s^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{min}}=\min\left(\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha}\right)-\bm{A}\delta\bm{x}^{\alpha}\right)\geq 0
\end{equation}
and $r^{\left\{\left\lvert\alpha\right\rvert+1\right\}}_{\mathrm{\max}}$ the maximum value of $\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha+1}\right)$
\begin{equation}
r^{\left\{\left\lvert\alpha\right\rvert+1\right\}}_{\mathrm{max}}=\max\left(\mathrm{cvx}\left(\bm{A}\delta\bm{x}^{\alpha+1}\right)\right)
\end{equation}
it is sufficient to show that within the trust region
\begin{equation}
s^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{min}} \geq r^{\left\{\left\lvert\alpha\right\rvert+1\right\}}_{\mathrm{max}}
\end{equation}
The smallest overestimation value $s^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{min}}$ within the trust region is
\begin{equation}
s^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{min}}=\min\left(a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{cvx},i}\right)\rho^{\left\lvert\alpha\right\rvert}.
\end{equation}
and within the trust region the maximum value is
\begin{equation}
r^{\left\{\left\lvert\alpha\right\rvert+1 \right\}}_{\mathrm{max}}=\max\left(\left\lvert a^{\left\{\left\lvert\alpha\right\rvert+1 \right\}}_{\mathrm{diag},i}\right\rvert+a^{\left\{\left\lvert\alpha\right\rvert+1 \right\}}_{\mathrm{cvx},i}\right)\rho^{\left\lvert\alpha\right\rvert+1}.
\end{equation}
Therefore trust region radius can be defined as 
\begin{equation}
\rho^{\left\{\left\lvert\alpha\right\rvert \right\}}=\frac{\min\left(a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{cvx},i}\right)}{\max\left(\left\lvert a^{\left\{\left\lvert\alpha\right\rvert+1 \right\}}_{\mathrm{diag},i}\right\rvert+a^{\left\{\left\lvert\alpha\right\rvert+1 \right\}}_{\mathrm{cvx},i}\right)}
\end{equation}
In principle, this trust region only guarantees that the inner convex approximations properties are maintained with respect to the following higher order term, $\alpha+1$. Yet, if it can be shown that the trust regions increase as the expansion order increases,
\begin{equation}
\rho^{\left\{\left\lvert\alpha\right\rvert \right\}}\leq \rho^{\left\{\left\lvert\alpha\right\rvert+1 \right\}}\leq \rho^{\left\{\left\lvert\alpha\right\rvert+2 \right\}}\leq\ldots
\end{equation}
then the convex inner approximation properties are guaranteed with respect to all higher order terms. 

\begin{comment}


. In order to truncate the series, while satisfying the properties in Eq~\eqref{eq:ConvexProp} and thus safeguarding the convergence properties that are derived from them, $n$ $L_{1}$ trust regions are enforced:
\begin{equation}
\left\lvert \delta x_{i}\right\rvert\leq\rho_{x_{i}}.
\end{equation}
The trust region size $\rho_{x_{i}}$ for each variable $x_{i}$ is determined as the difference from which the next higher-order term would surpass the last convexified term used:
\begin{equation}
a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{cvx}}\left\lvert \delta x^{\left\lvert\alpha\right\rvert}_{i}\right\rvert=a^{\left\{\left\lvert\alpha\right\rvert+1 \right\}}_{\mathrm{cvx}}\left\lvert \delta x^{\left\lvert\alpha\right\rvert+1}_{i}\right\rvert
\end{equation}
\begin{equation}
a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{cvx}} \rho^{\left\lvert\alpha\right\rvert}_{x_{i}}=a^{\left\{\left\lvert\alpha\right\rvert+1 \right\}}_{\mathrm{cvx}}\rho^{\left\lvert\alpha\right\rvert+1}_{x_{i}}
\end{equation}
\begin{equation}
\rho_{x_{i}}=\frac{a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{cvx}}}{a^{\left\{\left\lvert\alpha\right\rvert+1 \right\}}_{\mathrm{cvx}}}
\end{equation}
Inside the trust region the inequality
\begin{equation}
a^{\left\{\left\lvert\alpha\right\rvert \right\}}_{\mathrm{cvx}}\left\lvert x^{\left\lvert\alpha\right\rvert}_{i}\right\rvert\geq a^{\left\{\left\lvert\alpha\right\rvert+1 \right\}}_{\mathrm{cvx}}\left\lvert x^{\left\lvert\alpha\right\rvert+1}_{i}\right\rvert
\end{equation}
is satisfied and thus, the conditions defined in Eq.~\eqref{eq:ConvexProp} continue to hold.
\end{comment}

==> Variations.tex <==
Two particular implementations of the SCP are now briefly discussed as they have been used in trajectory optimization problems.

\subsection{Convex-concave procedure \label{sec:ccp}}
A convex-concave procedure \cite{Yuille2003,Lipp2016} is an SCP procedure where the non-convex functions $g_{i}$ are expressed as the difference of two convex functions $c\left(\bm{x}\right):\mathbb{R}^{n}\rightarrow\mathbb{R}$,
\begin{equation}
g_{i}\left(\bm{x}\right)=c_{i,1}\left(\bm{x}\right)-c_{i,2}\left(\bm{x}\right).
\label{eq:dc}
\end{equation}
Obtaining a convex inner approximation of a difference of convex function, a d.c. function in the sequel, is simple. The convex component, $c_{i,1}\left(\bm{x}\right)$, is kept as is, while the concave component, $-c_{i,2}\left(\bm{x}\right)$, is just linearized:
\begin{subequations}
\begin{equation}
	g^{\left(\bm{x}_{e}\right)}_{\text{cvx},i}\left(\bm{x}\right)=c_{i,1}\left(\bm{x}\right)-c_{i,2}\left(\bm{x}_{e}\right)-\delta\bm{x}^{T}\nabla c_{i,2}\left(\bm{x}_{e}\right).
	\label{eq:cccp}
\end{equation}
\begin{equation}
\delta\bm{x}=\bm{x}-\bm{x}_{e},
\end{equation}
\end{subequations}
As $g^{\left(\bm{x}_{e}\right)}_{\text{cvx},i}$ in Eq.~\eqref{eq:cccp} is a convex inner approximations satisfying the conditions in Eq.~\eqref{eq:ConvexProp}, the convex-concave procedure is a recursive feasible and convergent SCP \cite{Yuille2003,Lipp2016}.
 
Problem formulations with d.c. functions naturally appear in many optimization problems \cite{Tuy1995,Tao2005}, including in trajectory optimization, specially in the form of keep-out zone constraints \cite{Morgan2016,Liu2014,Debrouwere2013,Virgili2018_IJRR}. Keep-out zones are usually formulated as concave inequality constraints (\emph{i.e.}, a d.c. with $c_{i,1}\left(\bm{x}\right)=0$), and it appears that some authors have re-discovered that linearizing the concave constraints (or cost) yields a recursively feasible and convergent SCP procedure \cite{Morgan2016,Liu2014,Virgili2018_IJRR}.

\subsection{Successive linearization \label{sec:Suc_linear}}


==> ccp.tex <==
The convex-concave procedure \cite{Yuille2003,Lipp2016} is a class of SCP where any non-convex function $f$ is expressed as the difference of two convex functions $c_{1}\left(x\right),c_{2}\left(x\right):\mathbb{R}^{n}\rightarrow\mathbb{R}$,
\begin{equation}
f\left(x\right)=c_{1}\left(x\right)-c_{2}\left(x\right).
\label{eq:dc}
\end{equation}
Obtaining an inner-convex approximation of a difference of convex function, a d.c. function in the sequel, is simple. The convex component, $c_{1}\left(x\right)$, is kept as is, while the concave component, $-c_{2}\left(x\right)$, is just linearized:
\begin{equation}
	f^{\left(x_{e}\right)}_{\text{cvx}}\left(x\right)=c_{1}\left(x\right)-c_{2}\left(x_{e}\right)-\delta x^{T}\nabla c_{2}\left(x_{e}\right).
	\label{eq:cccp}
\end{equation}
The $f^{\left(x_{e}\right)}_{\text{cvx}}$ approximation in Eq.~\eqref{eq:cccp} is an inner-convex approximation and thus it follows that the convex-concave procedure is a recursively feasible and convergent \cite{Yuille2003,Lipp2016}.
 
Problem formulations with d.c. functions naturally appear in many optimization problems \cite{Tuy1995,Tao2005}.  A common example in trajectory optimization problems are keep-out zones, which are usually formulated as concave inequality constraints (\emph{i.e.}, a d.c. with $c_{1}\left(x\right)=0$). In these cases, linearizing the keep-out zone constraint yields a recursively feasible and convergent SCP procedure \cite{Morgan2016,Liu2014,Virgili2018_IJRR}.

It has been shown that d.c. decompositions exist for any twice differentiable function $f\in\mathcal{C}^{2}$  \cite{Hartman1959,Hiriart1985}. The convex-concave procedure is therefore applicable to a wide range of problems. 
The challenge then becomes: How do we find a d.c. decomposition?

%Simple function compositions, not apparently d.c., may be expressed as d.c. with the help of a few rules (see \cite{Hiriart1985,Wang2012b,Scutari2014} for more details).


\subsection{Regularization \label{sec:dc}}
The regularization approach is a general method to find d.c. decompositions \cite{Hiriart1985,Aleksandrov2012,Dinh2012,Wang2012b,Scutari2014}. In a regularization, a d.c. decomposition is obtained by using a sufficiently strong convex function $\phi\left(x\right):\mathbb{R}^{n}\rightarrow\mathbb{R}$ such that
\begin{equation}
f\left(x\right)=\underbrace{ \phi\left(x\right)}_{c_{1}\left(x\right)}-\underbrace{\left(\phi\left(x\right)-f\left(x\right)\right)}_{c_{2}\left(x\right)},\text{ for }x\in\mathcal{T},
\label{eq:regularization}
\end{equation}
is d.c in the trust region $\mathcal{T}$.%Ensuring that $x\in\mathcal{T}$ can be enforced with a trust region. 

Convex functions $\phi\left(x\right)$ where the convexity of $c_{2}=\phi\left(x\right)-f\left(x\right)$ can be rigorously proved may be difficult to obtain. However, if the $f$ function is Lipschitz continuous on $x\in\mathcal{T}$, with $K$ denoting the Lipschitz constant, a d.c. representation of $f$ over $\mathcal{T}$ is 
\begin{equation}
f\left(x\right)=\underbrace{K\left\lVert x\right\rVert^{2}}_{c_{1}\left(x\right)}-\underbrace{\left(K\left\lVert x\right\rVert^{2}-f\left(x\right)\right)}_{c_{2}\left(x\right)},\text{ for }x\in\mathcal{T}.
\end{equation}
The inner-convex approximation is then
\begin{equation}
f^{\left(x_{e}\right)}_{\text{cvx}}\left(x\right){=}f\left(x_{e}\right){+}\left(x{-}x_{e}\right)^{T}\nabla f\left(x_{e}\right){+}K\left\lVert x{-}x_{e}\right\rVert^{2}.
\end{equation}
The Lipschitz constant $K$ may not be known \textit{a priori}, but it can be estimated by $M> 0$. The inner-convex approximation candidate then becomes
\begin{equation}
f^{\left(x_{e}\right)}_{\text{cvx}}\left(x,M\right){=}f\left(x_{e}\right){+}\left(x{-}x_{e}\right)^{T}\nabla f\left(x_{e}\right){+}M\left\lVert x{-}x_{e}\right\rVert^{2}.
\end{equation}
The convex problem that uses these inner-convex approximations candidates, $P_{\mathrm{cvx}}^{\left(k\right)}\left(M\right)$ is then solved, and if the inner-convex properties of Eq.~\eqref{eq:ConvexProp_geq} are not met, chiefly if
\begin{equation}
f_{\mathrm{cvx}}^{\left(k-1\right)}\left(x_{\left(k\right)},M\right)< f\left(x_{\left(k\right)}\right),
\label{eq:Inner_convex_reg_1st_estimate}
\end{equation}
the convex problem is re-solved with a larger $M$, for example with $M_{\mathrm{new}}=\kappa M_{\mathrm{old}}$, with $\kappa> 1$. Problem $P_{\mathrm{cvx}}^{\left(k\right)}\left(M\right)$ is re-solved with increasingly larger $M$ until $f_{\mathrm{cvx}}^{\left(k-1\right)}\left(x_{\left(k\right)},M\right)\geq f\left(x_{\left(k\right)}\right)$. This sequence will not be infinite as eventually $M\geq K$ and thus the inner-convex candidate in Eq.~\eqref{eq:Inner_convex_reg_1st_estimate} will become an inner-convex approximation.

Following this principle, inner-convex approximations based on higher-order regularizations are also possible. For example, \cite{Nesterov2006} introduces a cubic regularization that enjoys a quadratic rate of convergence. But before we can present this approach some additional notation needs to be introduced.

Let the spectrum of a of an $n\times n$ symmetric matrix $\bm{A}$ be denoted by $\left\{\lambda_{i}\left(\bm{H}\right)\right\}_{i=1}^{n}$. Also, let's assume that the eigenvalues are ordered in a decreasing sequence:
\begin{equation}
\lambda_{1}\left(\bm{A}\right)\geq\ldots\geq\lambda_{n}\left(\bm{A}\right),
\end{equation}
and that the norm of a real symmetric matrix is defined with its standard spectral form as
\begin{equation}
\left\lVert\bm{A}\right\rVert=\sqrt{\lambda_{1}\left(\bm{A}^{T}\bm{A}\right)}.
\end{equation}
With these additional definitions, now suppose that the Hessian $\bm{H}\left(x\right)\in\mathbb{R}^{n\times n}$ of a non-convex function $f\left(x\right)$ is 
Lipschitz continuous on $x\in\mathcal{T}$, such that
\begin{equation}
\left\lVert\bm{H}\left(x_{1}\right)-\bm{H}\left(x_{2}\right)\right\rVert\leq K\left\lVert x_{1}-x_{2}\right\rVert,\text{ for }x\in\mathcal{T}.
\end{equation}
Then an inner-convex approximation of $f$ can be obtained by adding a cubic regularization to a second-order expansion as follows:
\begin{equation}
\begin{split}
f^{\left(x_{e}\right)}_{\text{cvx}}\left(x\right)=f\left(x_{e}\right)&+\left(x-x_{e}\right)^{T}\nabla f\left(x_{e}\right)\\
&+\frac{1}{2}\left(x-x_{e}\right)^{T}\frac{\bm{H}\left(x_{e}\right)}{2}\left(x-x_{e}\right)\\
&+\frac{K}{6}\left\lVert x-x_{e}\right\rVert^{3}.
\end{split}
\end{equation}
If $K$ is not known \emph{a priori}, it can also be estimated it with $M>0$. If the solution to the convex problem~$P_{\mathrm{cvx}}^{\left(k\right)}\left(M\right)$ doesn't meet $f_{\mathrm{cvx}}^{\left(k-1\right)}\left(x_{\left(k\right)},M\right)\geq f\left(x_{\left(k\right)}\right)$, $M$ is increased and the convex problem re-solved until the condition $f_{\mathrm{cvx}}^{\left(k-1\right)}\left(x_{\left(k\right)},M\right)\geq f\left(x_{\left(k\right)}\right)$ is met. 

With this approach, finding sufficiently strong regularizations can take several convex iterations and, when found, they might significantly overestimate $f$ and thus degrade the SCP procedure's rate of convergence.
It is also worth noting that infinite d.c. decompositions of $f$ exist (\emph{e.g.}, $\kappa K$ with $\kappa>1$ also yields a valid decomposition). Therefore, we are presented with the following question. Which is the ``best" inner-convex approximation of $f$? Inner-convex approximations that minimally overestimate $f$ may offer faster rates of convergence and are thus preferred. 

\subsection{Sum-of-squares decompositions}
An approach that is able to encode our desire to minimally overestimate $f$ is a d.c decomposition made by convex sum-of-squares polynomials (sos-convex in the following) \cite{Ahmadi2017}. Suppose that $f$ is a polynomial of degree $d_{f}$, and let $z\left(x\right)$ denote a vector of all the monomials of $x$ up to degree $d_{z}\geq d_{f}/2$. The sos-convex decomposition of $f$ is
\begin{equation}
\underbrace{z^{T}\bm{Q}_{f}z}_{f\left(x\right)}=\underbrace{z^{T}\bm{Q}_{1}z}_{c_{1}\left(x\right)}-\underbrace{z^{T}\bm{Q}_{2}z}_{c_{2}\left(x\right)},
\label{eq:sos}
\end{equation}
with $\bm{Q}_{f}$, $\bm{Q}_{1}$ and $\bm{Q}_{2}$ denoting real symmetric matrices containing the polynomial coefficients. %(also known as Gram matrices).
For the decomposition to be sos-convex and thus d.c., $\bm{Q}_{1}$ and $\bm{Q}_{2}$ must be positive semi-definite.
\begin{subequations}
\begin{equation}
f\left(x\right)=z^{T}\bm{Q}_{1}z-z^{T}\bm{Q}_{2}z
\end{equation}
\begin{equation}
\begin{rcases}
\bm{Q}_{1}\succeq 0 \Longrightarrow z^{T}\bm{Q}_{1}z\text{ is sos-convex}\\
\bm{Q}_{2}\succeq 0 \Longrightarrow z^{T}\bm{Q}_{2}z\text{ is sos-convex}
\end{rcases}
\Rightarrow f\text{ is d.c.}
\end{equation}
\end{subequations}
There are infinite sos-convex representations and thus in \cite{Ahmadi2017} different methods to optimize the sos-convex decomposition for a faster rate of convergence are proposed. Interestingly enough, finding these optimized sos-convex decompositions is a semidefinite programming problem (second order cone or linear programming problem with some additional relaxations) \cite{Ahmadi2017}. It is also worth noting that this approach has wide applicability, as any analytic function $f$ can be converted into polynomial form via a Taylor series expansion. Additionally, it is worth highlighting that the sos-convex decomposition approach is deeply connected to Laserre's approach in which sos-convex relaxations are used to cast non-convex polynomial programing problems as semidefinite programming problems \cite{Lasserre2001,Nie2013}.

The dimensionality of the semidefinite programming problem that needs to be solved to obtain these sos-convex decompositions dramatically increases with the number of constraints and variables. The practicality of the sos-convex decomposition is thus effectively limited to small problems with a limited number of variables and constraints. 

Up to this point, we have shown that inner-convex approximations for d.c. functions are easy to obtain. However, if the function is not d.c., either a semidefinite program needs to be solved to obtain a sos-convex decomposition or, for a regularization-based approximations, we need to estimate the Lipschitz constant, $M\geq K$ (potentially requiring to re-solve the convex problem multiple times). Therefore, obtaining an inner-convex approximations for non d.c. functions can be computational intensive, slowing down the SCP procedure.

